Structure-aware Fine-tuning of Sequence-to-sequence Transformers for Transition-based AMR Parsing

Predicting linearized Abstract Meaning Representation (AMR) graphs using pre-trained sequence-to-sequence Transformer models has recently led to large improvements on AMR parsing benchmarks. These parsers are simple and avoid explicit modeling of structure but lack desirable properties such as graph well-formedness guarantees or built-in graph-sentence alignments. In this work we explore the integration of general pre-trained sequence-to-sequence language models and a structure-aware transition-based approach. We depart from a pointer-based transition system and propose a simplified transition set, designed to better exploit pre-trained language models for structured fine-tuning. We also explore modeling the parser state within the pre-trained encoder-decoder architecture and different vocabulary strategies for the same purpose. We provide a detailed comparison with recent progress in AMR parsing and show that the proposed parser retains the desirable properties of previous transition-based approaches, while being simpler and reaching the new parsing state of the art for AMR 2.0, without the need for graph re-categorization.

==> figure2.tex <==
\begin{figure*}
    \centering
\hspace{-1cm}
\begin{tikzpicture}

% Aligned graph
%
\node [draw,rounded corners,thick] (you) at (1, 3) {\footnotesize you};
\node [] (token0) at (1,1) {\footnotesize You};
\path (token0) edge[-,draw,dashed,thick] (you);
\node [] (action0) at (1, 0) {\footnotesize $\cp$};
\node [] (pos0) at (1, 0.5) {\footnotesize 0};
\node [] (action1) at (2, 0) {\footnotesize $\shift$};
\node [] (pos1) at (2, 0.5) {\footnotesize 1};
%
\node [] (action2) at (3, 0) {\footnotesize tell};
\node [] (pos2) at (3, 0.5) {\footnotesize 2};
\node [] (action3) at (4, 0) {\footnotesize 01};
\node [] (pos3) at (4, 0.5) {\footnotesize 3};
\node [] (action4) at (4, -0.5) {\footnotesize $\la{0,arg0}$};
\node [] (action4b) at (5, 0) {\footnotesize $\textrm{ROOT}$};
\node [] (pos4b) at (5, 0.5) {\footnotesize 4};
\node [] (action5) at (6, 0) {\footnotesize $\shift$};
\node [] (pos5) at (6, 0.5) {\footnotesize 5};
%
\node [draw,rounded corners,thick] (tell) at (3, 4) {\footnotesize tell-01};
\node [] (token1) at (3,1) {\footnotesize told};
\path (token1) edge[-,draw,dashed,thick] (tell);
%
\node [draw,rounded corners,thick] (i) at (7, 2) {\footnotesize I};
\node [] (token2) at (7,1) {\footnotesize me};
\path (token2) edge[-,draw,dashed,thick] (i);
\node [] (action6) at (7, 0) {\footnotesize I};
\node [] (pos6) at (7, 0.5) {\footnotesize 6};
\node [] (action7) at (7, -0.5) {\footnotesize $\ra{1,arg1}$};
\node [] (action8) at (8, 0) {\footnotesize $\shift$};
\node [] (pos8) at (8, 0.5) {\footnotesize 8};
%
\node [] (token3) at (9,1) {\footnotesize to};
\node [] (action9) at (9, 0) {\footnotesize $\shift$};
%
\node [draw,rounded corners,thick] (watch) at (10, 3) {\footnotesize watch-01};
\node [] (token4) at (10,1) {\footnotesize watch};
\path (token4) edge[-,draw,dashed,thick] (watch);
\node [] (pos4) at (10, 0.5) {\footnotesize 3};
\node [] (action10) at (10, 0) {\footnotesize watch};
\node [] (action11) at (11, 0) {\footnotesize 01};
\node [] (action12) at (11, -0.5) {\footnotesize $\ra{1,arg1}$};
\node [] (action13) at (11, -1) {\footnotesize $\la{2,arg1}$};
\node [] (action14) at (12, 0) {\footnotesize $\shift$};
%
\node [] (token5) at (13,1) {\footnotesize the};
\node [] (action15) at (13, 0) {\footnotesize $\shift$};
%
\node [draw,rounded corners,thick] (dog) at (14, 2) {\footnotesize dog};
\node [] (token6) at (14,1) {\footnotesize dog};
\path (token6) edge[-,draw,dashed,thick] (dog);
\node [] (pos5) at (14, 0.5) {\footnotesize 4};
\node [] (action16) at (14, 0) {\footnotesize $\cp$};
\node [] (action12) at (14, -0.5) {\footnotesize $\ra{3,arg1}$};
% edges
\draw [->] (tell) to node[right] {{\footnotesize arg0}} (you);
\draw [->] (tell) to node[right] {{\footnotesize arg2}} (i);
\draw [->] (tell) to node[right] {{\footnotesize arg1}} (watch);
\draw [->] (watch) to node[right] {{\footnotesize arg0}} (i);
\draw [->] (watch) to node[right] {{\footnotesize arg1}} (dog);

% Action Sequence 
%\node [] (sentence) at (1, 0) {\footnotesize $\cp$ $\shift$ tell 01 $\cdots$};

\vspace{1cm}

\end{tikzpicture}

%\vspace{-0.2cm}
\caption{From top to bottom: Graph, sentence (source) and action sequence (target) for the sentence \textit{You told me to watch the dog} aligned to its AMR graph. AMR graph is displayed aligned to the source sentence. Arc-creating actions are displayed vertically due to space constraints.}
    \label{fig:graph_orders}
\end{figure*}


==> figure3_2.tex <==
\begin{figure*}
    \centering
%\hspace{-1cm}
\begin{tikzpicture}

%\def\actions{{"employ","01","person","$\shift$"}}%
%\foreach \i in {0,...,3} {%
%  \node [] (token\i) at ({1.2 * \i}, 1) {\pgfmathparse{\actions[\i]}\pgfmathresult};}

\def \xwarp {1.1}
\def \yposa {1}

\def \xpos {1}
% employ-01
\node [] (action) at ({\xpos * \xwarp}, 0.5) {\footnotesize 1};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize person};
\node [] (token) at ({\xpos * \xwarp},1) {\footnotesize Employees};
\node [draw,rounded corners,thick] (employee01) at ({\xpos * \xwarp}, 2) {\footnotesize employ-01};
\path (token) edge[-,draw,dashed,thick] (employee01);
\node [draw,rounded corners,thick] (person) at ({\xpos * \xwarp}, 3) {\footnotesize person};
\draw [<-] (employee01) to node[right] {{\footnotesize arg1-of}} (person);

\def \xpos {2.2}
% person
\node [] (action) at ({\xpos * \xwarp}, 0.5) {\footnotesize 2};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize employ-01};
\node [] (arc\xpos) at ({\xpos * \xwarp}, -0.5) {\footnotesize $\textsc{ra(1,arg1-\textup{of})}$};

\def \xpos {3.3}
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize $\textsc{shift}$};

\def \xpos {4.3}
% like-01
\node [] (action) at ({\xpos * \xwarp}, 0.5) {\footnotesize 5};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize like-01};
\node [] (token) at ({\xpos * \xwarp},1) {\footnotesize liked};
\node [draw,rounded corners,thick] (like01) at ({\xpos * \xwarp}, 4) {\footnotesize like-01};
\path (token) edge[-,draw,dashed,thick] (like01);
\draw [<-] (person) to node[right] {{\footnotesize \textsc{arg0}}} (like01);
\node [] (arc\xpos) at ({\xpos * \xwarp}, -0.5) {\footnotesize $\textsc{la(1,arg0)}$};

\def \xpos {5.3}
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize \textsc{root}};

\def \xpos {6.3}
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize $\textsc{shift}$};

\def \xpos {7.3}
\node [] (token) at ({\xpos * \xwarp},1) {\footnotesize their};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize $\textsc{shift}$};

\def \xpos {8.3}
% city
\node [] (action) at ({\xpos * \xwarp}, 0.5) {\footnotesize 10};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize city};
\node [draw,rounded corners,dashed,thick] (boston) at ({\xpos * \xwarp}, 1) {\footnotesize Boston};
\node [draw,rounded corners,thick] (name) at ({\xpos * \xwarp}, 2) {\footnotesize name};
\draw [<-] (boston) to node[right] {{\footnotesize op1}} (name);
\node [draw,rounded corners,thick] (city) at ({\xpos * \xwarp}, 3) {\footnotesize city};
\draw [<-] (name) to node[right] {{\footnotesize name}} (city);

\def \xpos {9.3}
% name
\node [] (action) at ({\xpos * \xwarp}, 0.5) {\footnotesize 11};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize name};
\node [] (arc\xpos) at ({\xpos * \xwarp}, -0.5) {\footnotesize $\textsc{ra(10,\textup{name})}$};

\def \xpos {10.9}
% COPY
\node [] (action) at ({\xpos * \xwarp}, 0.5) {\footnotesize 13};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize $\textsc{copy}$};
\node [] (arc\xpos) at ({\xpos * \xwarp}, -0.5) {\footnotesize $\textsc{ra(11,\textup{op1})}$};

\def \xpos {11.9}
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize $\textsc{shift}$};

\def \xpos {12.9}
% trip-03
\node [] (action) at ({\xpos * \xwarp}, 0.5) {\footnotesize 16};
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize trip-03};
\node [] (token) at ({\xpos * \xwarp},1) {\footnotesize trip};
\node [draw,rounded corners,thick] (trip03) at ({\xpos * \xwarp}, 3.5) {\footnotesize trip-03};
\path (token) edge[-,draw,dashed,thick] (trip03);
\draw [<-] (person) to node[right] {{\footnotesize \textsc{arg0}}} (trip03);
\draw [<-] (city) to node[right] {{\footnotesize \textsc{arg1}}} (trip03);
\draw [->] (like01) to node[right,bend left=30] {{\footnotesize \textsc{arg1}}} (trip03);
% arc actions
\node [] (arc\xpos) at ({\xpos * \xwarp}, -1) {\footnotesize $\textsc{ra(5,arg1)}$};
\node [] (arc\xpos) at ({\xpos * \xwarp}, -1.5) {\footnotesize $\textsc{la(1,arg0)}$};
\node [] (arc\xpos) at ({\xpos * \xwarp}, -0.5) {\footnotesize $\textsc{la(10,arg1)}$};

\def \xpos {13.9}
\node [] (action) at ({\xpos * \xwarp}, 0) {\footnotesize $\textsc{shift}$};

\end{tikzpicture}

\vspace{-2mm}
\caption{From top to bottom: graph, sentence (source), addressable action positions and action sequence (target) for the sentence \textit{Employees liked their Boston trip}, aligned to its AMR graph. Arc-creating actions are displayed vertically due to space constraints. LA(1,ARG0) creates an edge (Left-Arc) from root concept \textit{like-01} to the concept generated in position 1 \textit{person} with label ARG0. For concept \textit{trip-03}, LA(1,ARG0) is a co-reference (re-entrancy) for the subject \textit{person}. COPY action in postion 13 indicates copying the input token \textit{Boston}.
%Separate vocabulary strategy used, see Section \ref{sec:exp_setup}.
}
    \label{fig:graph_orders}
\end{figure*}

